Topological Data Analysis of copy number alterations in cancer

Identifying subgroups and properties of cancer biopsy samples is a crucial step towards obtaining precise diagnoses and being able to perform personalized treatment of cancer patients. Recent data collections provide a comprehensive characterization of cancer cell data, including genetic data on copy number alterations (CNAs). We explore the potential to capture information contained in cancer genomic information using a novel topology-based approach that encodes each cancer sample as a persistence diagram of topological features, i.e., high-dimensional voids represented in the data. We find that this technique has the potential to extract meaningful low-dimensional representations in cancer somatic genetic data and demonstrate the viability of some applications on finding substructures in cancer data as well as comparing similarity of cancer types.

==> Figures/heatmap.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tbp]
    \centering
        %
        \includegraphics[width=0.7\linewidth]{Figures/images/Diagrams_cosine_normalized_clustered_distancemetric_bottleneck_transform_None.pdf}
        %
    \caption{
        Heatmap depicting the \emph{bottleneck} distance between persistence diagrams of different cancer types. The persistence diagram calculated from the complete dataset, including all cancer types, is seen in \emph{pan-cancer}.
             }
    \label{fig:heatmap}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> preamble.tex <==
\PassOptionsToPackage{numbers, compress}{natbib}
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[british]{babel} % hyphenation patterns
\usepackage{csquotes}       % context-sensitive quotes
\usepackage{hyperref}       % hyperlinks
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsmath}        % basic mathematical typesetting
\usepackage{amssymb}        % basic mathematical symbols
\usepackage{amsthm}         % basic mathematical theorems
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{dsfont}         % proper double-stroke font for mathematics
\usepackage{graphicx}       % graphics
\usepackage{mathtools}      % additional tools for mathematical typesetting
\usepackage{microtype}      % microtypography
\usepackage{mleftright}     % ensures proper spacing for mathematical expressions
\usepackage{multirow}       % spanning multiple columns and rows in tables
\usepackage{nicefrac}       % better inline fractions
\usepackage{paralist}       % for in-paragraph lists
\usepackage{subcaption}     % sub-captions for figures
\usepackage{siunitx}        % SI units and number typesetting
\usepackage{url}            % simple URL typesetting
\usepackage{xspace}         % fix spacing-related issues
\usepackage{xcolor}
% \usepackage{microtype}      % tightens layout

\newcommand{\diagram} {\mathcal{D}}
\newcommand{\manifold}{\mathcal{M}}

\newcommand{\reals}   {\mathds{R}}

\DeclareMathOperator{\vietoris}{\mathfrak{V}}

\usepackage{array, makecell}
\graphicspath{ {Figures/} }
\usepackage[inline]{enumitem}
\setlist[enumerate,1]{label=\textit{\alph*)}}
\usepackage{hyperref}


\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=blue,
}

\usepackage{pgfplots}          % plots
\usepackage{tikz}              % more plots

\usetikzlibrary{calc}

\definecolor{cardinal}{RGB}{196, 30, 58}
\definecolor{bleu}    {RGB}{ 49,140,231}


% This is required for Overleaf because they do not support more recent
% versions of `pgfplots` at present.
\pgfplotsset{compat=1.16}

\usepgfplotslibrary{colorbrewer}
\usepgfplotslibrary{fillbetween}
\usepgfplotslibrary{groupplots}

\usepackage[subrefformat=parens]{subcaption}

